Design and Evaluation of IPFS: A Storage Layer for the Decentralized Web

Recent years have witnessed growing consolidation of web operations. For example, the majority of web traffic now originates from a few organizations, and even micro-websites often choose to host on large pre-existing cloud infrastructures. In response to this, the "Decentralized Web" attempts to distribute ownership and operation of web services more evenly. This paper describes the design and implementation of the largest and most widely used Decentralized Web platform - the InterPlanetary File System (IPFS) - an open-source, content-addressable peer-to-peer network that provides distributed data storage and delivery. IPFS has millions of daily content retrievals and already underpins dozens of third-party applications. This paper evaluates the performance of IPFS by introducing a set of measurement methodologies that allow us to uncover the characteristics of peers in the IPFS network. We reveal presence in more than 2700 Autonomous Systems and 152 countries, the majority of which operate outside large central cloud providers like Amazon or Azure. We further evaluate IPFS performance, showing that both publication and retrieval delays are acceptable for a wide range of use cases. Finally, we share our datasets, experiences and lessons learned.

==> archive/2.content-publishing.tex <==
\section{Publishing Content in IPFS}\label{content-publishing}

% \gareth{It feels like we are jumping into publishing before we have given a proper architectural overview of the system. Ideally, we could have a diagram revealing the main components and then each of these sections is linked into it?}
% \yiannis{Leaving the structure below largely as is, because after adding the architecture overview, it will (hopefully) all make sense.}
% \yiannis{In fact, I've moved the the description of the CID to the section above and left the rest here.}

We describe the steps involved in \textit{Content Publication}, which are: Importing \& Addressing (Section \hl{XX}) and Publication of a pointer (\textit{aka} Provider Record) to the IPFS network (Section \hl{XX}).
% When a user wishes to publish content in IPFS, they first need to \textit{add it to the file system}.

\gareth{General preference: I never think it's worthwhile starting sections with a list of the subsections. People can easily read that by looking at the subsection titles. Instead, it's better to use this as an opportunity to spin out the narrative of the section.}

% \subsection{Importing \& Addressing Content}

% When content is added/imported to the IPFS file system it is split into 256KB chunks. In turn, each chunk is given a unique address, the \textit{Content Identifier}, or CID, that results from hashing its content and adding metadata. Once all chunks have been addressed, IPFS constructs a Merkel-DAG of the file. \hl{+details on Merkle DAGs?+}
% % publishing content, IPFS first performs \textit{chunking}. This involves splitting the content into chunks of 256KB, and allocating each a unique address. Following this, a Merkel-DAG is constructed. 

% Given their hash-based structure, CIDs are permanent, immutable and self-certifying, which make them a great fit as a base layer for decentralized storage, but at the same time not very practical for everyday applications. In order to account for mutable content, IPFS provides the option of publishing content based on the hash of the publisher's public key (\ie PeerID), instead of the CID itself. This way, content can be updated (and obtain a different CID), but always point to the same peer, using the same resolution, discovery and routing system. For this reason, we leave further details out of this study and point the reader to \hl{[ipns], [dnslink]} for further details.

% \gareth{Feels lie the above is repeating what was in the previous section?}



\subsection{Adding the Provider Record to IPFS}
\label{sec:provider-records}

After chunking the object, addressing each of the chunks and constructing the Merkle-DAG, the IPFS client instance ``adds" the content to the IPFS network. The content is not replicated or uploaded to any external server. The content stays local on the user's device and instead, it is the Content Identifier (CID) together with a pointer to the user's machine that is made known to the network (in particular to the Content Routing component of the system - see Section~\ref{content-routing}). 
The user adding content is called a Content \emph{Provider} or \emph{Publisher}; and the record published to the routing system is the \textit{Provider Record}.

A provider record is stored to the 20 nodes that are closest in terms of XOR distance from the hash of the content being added to the network. 
%%%

\gareth{Add back of the envelope calc for 20 then revisit in evaluation}

A provider record is also added to the system when a user requests and retrieves content from the original content publisher. In this case, the content is cached on their device and they become temporary providers for the content. A method called ``garbage collection" eventually clears the cache of retrieved content [after 24hrs, or when storage reaches 10GBs], unless the user \textit{pins} it explicitly in which case it becomes a permanent provider (similar to the original content publisher).

\gareth{We should formally describe the provider record (i.e. the schema)}
\yiannis{Dennis, do you want to add the schema here and provide a brief description as needed?}

By default, the provider record is stored on 20 peers. This means that the failure of a single peer does not remove the record from the system. The 20 peers are chosen based on the hash-distance of their PeerID from the hash of the content itself (\ie CID). 
% To enable this, each peer in IPFS is allocated a unique identifier (\ie PeerID) that occupies the same hash space as the content identifiers.
% We discuss in more detail how provider records are assigned to peers in Section~\ref{libp2p-dht}.

Provider records contain two parameters that relate to their validity, both of which attempt to make the system more robust against network churn, and/or resource shortage (\ie in case a content publisher does not have enough resources to maintain previously published content items).

\begin{enumerate}
    \item \textbf{Re-publish interval:} This represents the period after which the publisher must re-publish the provider record and is set to 12 hours by default.\footnote{As we discuss in Section~\ref{libp2p-dht}, one of the ways this is done in IPFS is through a Distributed Hash Table (DHT).}. The re-publish interval is there to make sure that there are enough peers online to provide the record, \ie even if the peers previously responsible for keeping the provider record alive have gone offline, the provider will assign new ones within the next 12 hours.
    
    
    \item \textbf{Expiry interval:} during this interval, currently set to 24hrs, the original publisher has to re-provide all the records for the content it makes available to the network. This parameter is needed in order to make sure that: i) the publisher is still online and can provide the content, and ii) the collection of content items that the publisher is still making available to the network is accurate (\ie there are no stale records pointing to unavailable conten).\footnote{The publisher might have decided that they do not want to, or cannot (\eg due to resource constraints) provide some content items anymore.}. After the expiry of a provider record, peers that were responsible for keeping the provider record will not provide it to clients.
\end{enumerate}

In summary, the re-publish interval protects against provider records not being available in the network due to peer churn and the expiry interval protects against stale provider records when content publishers go offline, or are resource constrained.

% \gareth{Not sure I understand the nuance of the above two things. General point: We also tend to use bullet point lists a lot. These are great for emphasising the importance of a set of things. However, sometimes it feels like we are putting unimportant things in lists (with quite verbose text).}
% \yiannis{These settings are important to protect against peer churn. Maybe it's not clear due to the structure and flow of the paper in the previous section, but it will be in the next one. I believe they're important to keep. I don't mind removing the bullet point structure.}


The re-publication of provider records is very effective against network churn, although it imposes greater upstream bandwidth requirements for publisher peers. Recall that the ``importing and addressing'' process is assigning a CID to every content chunk. This means that every content chunk is an independent, directly identifiable object that can live together with the rest of the file, or not, and therefore, provider records have to be updated for every chunk. It is clear then that the size of content chunks becomes a trade-off between the granularity of serving individual chunks and the overhead of keeping state as well as republishing provider records per chunk. Larger content chunks incur less overhead (both to the peer that keeps state and the network that transmits less provider records) at the cost less fine-grained access to content.
\gareth{The above paragraph feels a bit 'rambly'. It generally discusses things but not in any depth, not does it reach a clear conclusion that has been factored into the design. I would perhaps delete...?}
\yiannis{Good point. What we should emphasize here is that this is an open issue that requires further attention. OTOH, a comment such as just publish the root CID of the file and not every CID of every 256KB-chunk is an easy one to make. So, I wouldn't mind deleting, but let's leave it to the next iteration:)}


==> archive/3.content-routing-arch.tex <==
\section{Retrieving Content from IPFS}\label{content-routing}

Retrieving content from IPFS is composed of three procedures: 
\one~Content Discovery;
\two~Peer Discovery;
and 
\three~Peer Routing. In this Section, we describe each one of these procedures in turn, but we start by giving some more details about IPFS's Distributed Hash Table (DHT), which serves as the most widely used resolution system of IPFS and the one of interest in this study.\footnote{It is important to highlight that the DHT is only one of the content routing subsystems provided by libp2p with alternatives, such as mDNS, js-ipfs, \hl{++}, being available and operational.}


% Peer Discovery \& Peer Routing are part of libp2p. Both Content \& Peer Discovery utilise libp2p's Distributed Hash Table (DHT). It is important to highlight that the DHT is only one of the content routing subsystems provided by libp2p with alternatives, such as mDNS, js-ipfs, \hl{++}, being available and operational. There are several libp2p protocols involved in the content resolution and delivery, such as techniques for NAT-Traversal and Stream Multiplexing \hl{[link to repos]}. Due to space limitations, here we will only refer to those components of libp2p that are essential for content resolution and delivery and provide links to the rest, where appropriate.



We now proceed to describe the three steps involved in content retrieval, namely, \one~Content Discovery;
\two~Peer Discovery;
and 
\three~Peer Routing.

\subsection{Content Discovery.} The libp2p DHT implements \textit{multi-round iterative lookups} in order to resolve a CID to a peer's multiadddress. When peer $x$ issues a request for CID $y$, the request is forwarded to $a=3$ \hl{[]} nodes whose PeerIDs are closest to $y$ in peer $x$'s routing table. The peers receiving those requests reply with the requested content object, if they have it. If they do not have the requested content item, they reply with either the provider record that points to the PeerID that holds the requested item together with the peer's multiaddress (if they have it), or the peers it knows of whose PeerID is closer to $y$. The process continues until the node is returned with the PeerID that has previously declared to hold a copy of the requested CID through a published provider record.

\subsection{Peer Discovery.} After the content discovery phase, the requesting peer knows the PeerID of the content (CID) it is looking for, but in many cases the requesting peer still does not know the multiaddress of the peer it needs to connect to. As mentioned earlier, PeerIDs in libp2p are multihashes and therefore, they have to be resolved to a physical network address. This procedure is called \emph{Peer Discovery}. If peer discovery has not taken place together with content discovery (\ie when the multiaddress is returned together with the PeerID), it is carried out by ``walking" the DHT for a second time.

\subsection{Peer Routing.} Once the PeerID is resolved through the second DHT walk, the requesting peer has obtained the multiaddress of the peer that appears to have the content. It therefore, uses this multiaddress to connect to and fetch the content.


\subsection{Bitswap: The Block Exchange Protocol}
\label{sec:bitswap}

Once a set of storage locations have been identified, the next step is for the client to download the segments. This is done using Bitswap, which is a simple chunk exchange protocol. 

% \gareth{Another quick pointer: this above paragraph doesn't actually start by explaining what Bitswap does. I've rewritten it now, but I've noticed this a few times. We start of a subsection introducing a new concept of compeonent. But we forget to actually explain what the component does or the role it plays in IPFS.}

Due to its simple design, Bitswap can, in certain cases, complete content and peer discovery faster than the DHT.
For this reason, Bitswap makes a content discovery attempt before the DHT actually kicks in.
Bitswap utilises the list of peers that a specific node is connected to.\footnote{IFPS nodes keep a long list of connected peers (up to \hl{900}), which is the list of all the peers that a node has ever seen, or interacted with. Apart from peers that belong to the node's DHT routing table, this list includes peers that do not fall into any of the peer's DHT routing table entries (\ie k-buckets).} 

When a client wants to retrieve a file from IPFS, it explicitly asks \textit{all of those connected peers} for the items it wants - this is the \textit{wantlist} of the peer in the Bitswap protocol. Requests are sent out using an \texttt{IWANT-HAVE} message which prompts those peers that have the block to reply with a corresponding \texttt{IHAVE} message. The requesting peer then responds with an \texttt{IWANT-BLOCK} message. Receipt of the requested block terminates the exchange. The full details of the Bitswap protocol design as well as a number of proposed optimizations can be found in \hl{[link to paper]}.

% There are a number of optimisations done to the above procedure in order to speed up content retrieval with Bitswap.

% \begin{enumerate}
% \item \textit{Peer Choice:} Choosing which peer to ask for the \texttt{IWANT-BLOCK} message is done probabilistically - \hl{add based on what?}
% \item \textit{Bitswap Sessions:} It is very likely that peers who have one block of an object have the rest of the blocks too. Therefore, Bitswap groups those peers who have replied with an \texttt{IHAVE} message into one \textit{session} and is asking those peers for the subsequent blocks of the content item only.
% \item \textit{Small Blocks:} In case of very small blocks \hl{(in the order of [size?])}, peers that receive an \texttt{IWANT-HAVE} message reply with the block itself, rather than an \texttt{IHAVE} message. This is to avoid an extra RTT.
% \end{enumerate}


% \subsection{Content Discovery \& Routing Summary}

% Summarising, the steps followed to discover content and fetch content in IPFS are as follows:
% \hl{[ideally show in figure too]}
% \begin{enumerate}
% \item Get CID (out of band)
% \item Broadcast the WANTLIST to all of the connected peers.
% \item If no IWANT-HAVE message is received proceed to DHT search.
% \item Walk the DHT to resolve CID to PeerID. The DHT will return the multiaddress in addition to the PeerID, if it has it.
% \item As a fallback in case the multiaddress is not returned together with the PeerID from the previous step: Walk the DHT again to get the multiaddress of the PeerID
% \item Contact PeerID to ask for content
% \item Fetch content using Bitswap by sending the WANTLIST to the PeerID and cache a copy
% \item Serve local copy upon subsequent request
% \end{enumerate}

% \gareth{I would remove this above list.}
% \yiannis{I still think it's valuable to show the sequence, but, as discussed, better do it in a figure and include upfront. Commenting out the subsection for now.}

==> archive/3.operation.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{IPFS in action}
\label{sec:ipfs_in_action}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

To make content available in the IPFS network it is \one imported to the IPFS file system and allocated a CID.
Then, the host \two pushes a \emph{provider record} into the libp2p DHT mapping the CID to its own PeerID.
Section~\ref{content-publishing} discusses the steps required to publish content.

Once the provider record has been published, users can retrieve the content. 
To retrieve the content the requesting peer \one identifies peer(s) that have declared to be willing to provide a copy of the content (\textit{content discovery}),
\two maps the PeerID to a Multiaddress, \eg an IP address, (\textit{peer discovery}),
and \three routes to the peer, by requesting and getting the content (\textit{peer routing} and \textit{content fetching}).
This process we call \textit{content retrieval} and Section~\ref{content-routing} details the steps involved.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Publishing content}
\label{content-publishing}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

When a user (\emph{publisher}) imports content into IPFS,
the content is not replicated or uploaded to any external server.
Instead, the  \emph{publisher} adds a \textit{provider record} to the routing system.
\ignacio{where do we define ``routing system''}

For resilience purposes,
this provider record is stored to the 20 closest nodes in terms of XOR distance from the hash of the content (\ie CID) added to the network. 
This prevents that the failure of a single peer does not remove the record from the system. 

% When a user imports content into IPFS, the content is split into 256KB chunks, each with a CID 
% After chunking the content, associating each chunk to its CID and constructing the Merkle-DAG, the IPFS client instance ``adds" the content to the IPFS network. 
% \ignacio{what is precisely the ``the IPFS network''. Can we define?}
% The content is not replicated or uploaded to any external server.
% The content stays local on the user's device and instead.
% Instead, it is the CID and a pointer to the user's machine that is made known to the network. 
% Instead, the user adding content, \ie the \emph{publisher}, adds a \textit{Provider Record} to the routing system.
% The provider record is stored to the 20 nodes that are closest in terms of XOR distance from the hash of the content (\ie CID) added to the network. 
% This means that the failure of a single peer does not remove the record from the system. 
%%%

\gareth{Add back of the envelope calc for 20 then revisit in evaluation}

IPFS also provides caching.
When a user retrieves content from the original publisher, the content is cached on the device of the user requesting the content who adds a provider record to the system and becomes a temporary provider of the content.
\ignacio{temporary: when does the node cease to provide the content?}
%
A user can however decide to become a  permanent provider of the content (like the publisher) by explicitly  \textit{pinning} the content.
\ignacio{do we need to define ``pinning''?}

A distributed system like IPFS faces the challenge of storing content in resource-constraint peers that might not always be online.
To prevent overloading the memory of the devices of the users and/or keeping stale provider records in the system, 
content publisher records expire (currently every 24hrs.).
%
During this interval, the original publisher has to re-provide all the provider records of the published content. \ignacio{during or every 24h?}
This serves to ensure that the publisher is available to provide the content (\ie is online), and that there are no stale records pointing to unavailable content (\eg because the publisher decides not to provide specific content anymore).
%
% After the expiry of a provider record, peers that were responsible for keeping the provider record will not provide it to clients.




% To prevent overloading the memory of the devices of the users, 
% a ``garbage collection'' mechanism clears the cache of retrieved content \hl{[after 24hrs, or when storage reaches 10GBs]}.
% A user can however decide to become a  permanent provider of the content (like the publisher) by explicitly  \textit{pinning} the content.
% \ignacio{do we need to define ``pinning''?}

% \textbf{Expiry interval:} during this interval, currently set to 24hrs, the original publisher has to re-provide all the records for the content it makes available to the network. This parameter is needed in order to make sure that: i) the publisher is still online and can provide the content, and ii) the collection of content items that the publisher is still making available to the network is accurate (\ie there are no stale records pointing to unavailable content).\footnote{The publisher might have decided that they do not want to, or cannot (\eg due to resource constraints) provide some content items anymore.} After the expiry of a provider record, peers that were responsible for keeping the provider record will not provide it to clients.

% A provider record is also added to the system when a user requests and retrieves content from the original content publisher. In this case, the content is cached on their device and they become temporary providers for the content. A method called ``garbage collection" eventually clears the cache of retrieved content \hl{[after 24hrs, or when storage reaches 10GBs]}, unless the user \textit{pins} it explicitly, in which case it becomes a permanent provider (similar to the original content publisher).

\gareth{We should formally describe the provider record (i.e. the schema)}
\yiannis{Dennis, do you want to add the schema here and provide a brief description as needed?}
\ignacio{PRovider record to be described at the end of the previous section?}

 
% To enable this, each peer in IPFS is allocated a unique identifier (\ie PeerID) that occupies the same hash space as the content identifiers.
% We discuss in more detail how provider records are assigned to peers in Section~\ref{libp2p-dht}.

Peer churn, common in peer-to-peer networks,  poses a a challenge to the availability of content.
To ensure that enough online peers have the content, 
the publisher recurrently re-publishes the provider record.
By default, the re-publishing interval is set to 12 hours.\footnote{As we discuss in Section~\ref{libp2p-dht}, one of the ways this is done in IPFS is through a Distributed Hash Table (DHT).\ignacio{how specifically is it done}}


The size of the content chunks provides a trade-off between the granularity of serving individual chunks and the overhead of keeping state as well as republishing provider records per chunk
\ignacio{this probably should be moved somewhere else}

% \begin{enumerate}
% 	\item \textbf{Re-publish interval:} This represents the period after which the publisher must re-publish the provider record and is set to 12 hours by default.\footnote{As we discuss in Section~\ref{libp2p-dht}, one of the ways this is done in IPFS is through a Distributed Hash Table (DHT).}. The re-publish interval is there to make sure that there are enough peers online to provide the record, \ie even if the peers previously responsible for keeping the provider record alive have gone offline, the provider will assign new ones within the next 12 hours.
	
	
% 	\item \textbf{Expiry interval:} during this interval, currently set to 24hrs, the original publisher has to re-provide all the records for the content it makes available to the network. This parameter is needed in order to make sure that: i) the publisher is still online and can provide the content, and ii) the collection of content items that the publisher is still making available to the network is accurate (\ie there are no stale records pointing to unavailable content).\footnote{The publisher might have decided that they do not want to, or cannot (\eg due to resource constraints) provide some content items anymore.} After the expiry of a provider record, peers that were responsible for keeping the provider record will not provide it to clients.
% \end{enumerate}

% In summary, the re-publish interval protects against \hl{provider records not being available in the network due to peer churn} and the expiry interval protects against stale provider records when content publishers go offline, or are resource constrained.

% \gareth{Not sure I understand the nuance of the above two things. General point: We also tend to use bullet point lists a lot. These are great for emphasising the importance of a set of things. However, sometimes it feels like we are putting unimportant things in lists (with quite verbose text).}
% \yiannis{These settings are important to protect against peer churn. Maybe it's not clear due to the structure and flow of the paper in the previous section, but it will be in the next one. I believe they're important to keep. I don't mind removing the bullet point structure.}


% The re-publication of provider records is very effective against network churn, although it imposes greater upstream bandwidth requirements for publisher peers. Recall that the ``importing and addressing'' process is assigning a CID to every content chunk. This means that every content chunk is an independent, directly identifiable object that can live together with the rest of the file, or not, and therefore, provider records have to be updated for every chunk. It is clear then that the size of content chunks becomes a trade-off between the granularity of serving individual chunks and the overhead of keeping state as well as republishing provider records per chunk. Larger content chunks incur less overhead (both to the peer that keeps state and the network that transmits less provider records) at the cost less fine-grained access to content.
% \gareth{The above paragraph feels a bit 'rambly'. It generally discusses things but not in any depth, not does it reach a clear conclusion that has been factored into the design. I would perhaps delete...?}
% \yiannis{Good point. What we should emphasize here is that this is an open issue that requires further attention. OTOH, a comment such as just publish the root CID of the file and not every CID of every 256KB-chunk is an easy one to make. So, I wouldn't mind deleting, but let's leave it to the next iteration:)}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Addressing Content}
% \begin{figure}
%     \centering
%     $
%     \underbrace{\overset{\texttt{v1}}{00000001}}_{\texttt{Version}}
%     \underbrace{\overset{\texttt{dag-pb}}{01110000}}_{\texttt{Multicodec}}
%     \underbrace{\underbrace{\overset{\texttt{sha2-256}}{00010010}}_{\texttt{Multicodec}}
%     \underbrace{\overset{\text{\texttt{32 bytes}}}{00100000}}_{\texttt{Length}}\underbrace{\overset{\texttt{SHA256 hash}}{110010010\dots}}_{\texttt{Actual Hash}}}_{\texttt{Multihash}}
%     $
%     \vspace{-0.3cm}
%     \caption{Binary representation of a CID.}
%     \label{fig:cid_binary}
% \end{figure}
% \ignacio{Not sure I get the logical difference between this subsection and the next one}

% Here, we describe our approach to addressing content, remote processes and peers. Our design goals of the addressing schemes are verifiability, forward compatibility, interoperability, and protocol agility to avoid lock in.
% \gareth{Minor point, but we should try to use the initial paragraph to fit the section into the overall narrative of the paper (rather than just listing the content of the section).}


% \pb{The Content Identifier (CID).} IPFS allocates a hash-based unique identifier to content that we call \textit{content identifier} or CID. CIDs follow a data representation standard\footnote{\url{https://multiformats.io/}}, which adds \textit{self-describing} attributes to the data. At the time of writing there are two CID versions. The following shows an example for both that identify the same content

% \begin{table}[H]
%     \centering
%     \scriptsize
%     \vspace{-0.4cm}
%     \begin{tabular}{ll}
%         \texttt{CIDv0} & \texttt{QmbWqxBEKC3P8tqsKc98xmWNzrzDtRLMiMPL8wBuTGsMnR} \\
%         \texttt{CIDv1} & \texttt{bafybeigdyrzt5sfp7udm7hu76uh7y26nf3efuylqabf3oclgtqy55fbzdi} \\
%     \end{tabular}
%     \vspace{-0.4cm}
% \end{table}

% \noindent In general, CIDs adhere to the following form:
% \begin{center}
%     \small
%     \vspace{0.1cm}
%     \texttt{<multibase>(cid-version~$\oplus$~multicodec~$\oplus$~multihash)}
%     \vspace{0.1cm}
% \end{center}
% \noindent Each of these parts serve a well-defined purpose:

% % \begin{figure}[t]
% % % \resizebox{0.8\columnwidth}{!}{
% % \begin{centering}
% % \small
% % $
% % \underbrace{\overbrace{\hbox{\texttt{<base>}}}^{\parbox{1cm}{\centering base32}}}_{\parbox{1cm}{Encoding}} 
% % \oplus \ \ \underbrace{\overbrace{\hbox{\texttt{cid-version}}}^{\parbox{1.8cm}{\centering v0 or v1}}}_{\hbox{CID Version Used}}\
% % \oplus \ \ \underbrace{\overbrace{\hbox{\texttt{multicodec}}}^{\parbox{1.5cm}{\centering 0x70}}}_{\hbox{\eg dag-pb}}\ 
% % \oplus \ \ \underbrace{\overbrace{\hbox{\texttt{multihash}}}^{\parbox{1.5cm}{\centering Qm...}}}_{\hbox{Hash + metadata}}\ 
% % $
% % \caption{Multiformats Structure \& Examples}
% % \label{fig:names}
% % \end{centering}
% % % }
% % \end{figure}
% % \pb{Multibase:} The identifier of the base-encoding used for the CID, \eg ``b" of base32, ``f" for base16. It denotes how the CID has been encoded and therefore, how to transform the CID to a binary format.

% % \pb{CID-version:} A field to denote different versions of CIDs. Currently there are two versions (v0 and v1), but this field is there for future needs of the architecture or applications.

% % \pb{Multicodec:} A unique number, which identifies a protocol, protocol version, hash-function, format, or even an arbitrary naming primitive. The list of (more than 400) current multicodecs is publicly available\footnote{\url{https://github.com/multiformats/multicodec/blob/master/table.csv}} and new multicodecs can be proposed.

% % \pb{Multihash:} A self-describing hash-digest with metadata to denote the length of the hash as well as the hash-function used (included as a \texttt{multicodec}).

% \begin{description}
%     \item[Multibase] The identifier of the base-encoding used for the CID, \eg ``b" of base32, ``f" for base16. It denotes how the CID has been encoded and therefore, how to transform the CID to a binary format. Currently, there are 24 supported base encodings available\footnote{\url{https://github.com/multiformats/multibase/blob/master/multibase.csv}}.
    
%     \item[CID-version] A field to denote different versions of CIDs. Currently there are two versions (v0 and v1), but this field is there for future needs of the architecture or applications.
    
%     \item[Multicodec] A field that identifies a protocol, protocol version, hash-function, format, or even an arbitrary naming primitive. The list of (more than 400) current multicodecs is publicly available\footnote{\url{https://github.com/multiformats/multicodec/blob/master/table.csv}}.
    
%     \item[Multihash] A self-describing hash-digest with metadata to denote the length of the hash as well as the hash-function used (included as a \texttt{multicodec}).
% \end{description}
% Figure~\ref{fig:cid_binary} shows the binary representation of a CID with all the components above. All parts, except the ``Actual Hash'', are encoded as variable size integers to future-proof the format.

% This use of self-describing digests is a core design decision, as it enables decentralized content address management without the need for any authority to handle allocation. It is a central component of decentralized network design, as it enables content being stored in any platform without it being ``locked" to a specific storage provider. This is in contrast to location-based identifiers, such as IP addresses, which bind content to its primary host. The hash-based CID further means that any changes to the content will inherently result in a different address. This means that hash-based identifiers enable \textit{self-certification}, that is, clients can easily verify content they received by comparing the requested identifier against the resulting hash of the content.
% \dennis{Mention de-duplication as another advantage?}

% \pb{The Multiaddress.} 
% libp2p defines the concept of ``Multiaddresses". It is used to address remote processes by encoding multiple blocks/layers of addressing information into a path representation. A \textit{Multiaddress} is a human-readable, hierarchically-separated sequence of protocol choices from the network-layer up to the application layer that are to be used in the interaction between two peers. For example, the \texttt{multiaddr: /ip4/1.2.3.4/tcp/3333} defines two protocols for this communication (IPv4 and TCP) with their corresponding addressing information (the actual IP address and TCP port number). \hl{mention and show byte-encoding in a figure?}

% \gareth{The above multiaddress definition is a bit confusing - not very clear what it does or why}

% \dennis{From the former ``Deployment Overview'' section 6.1 (not there anymore). We may keep the following in this section here: ``Note that a single Multiaddress can link to one or many IP addresses depending on the encoded protocols. For example, the \texttt{dnsaddr} Multiaddress protocol may resolve to a set of different Multiaddresses, each pointing to a different host with a unique IP address. However, the more frequent case is several Multiaddresses encoding the same IP address. Such Multiaddresses often only differ further down in the protocol hierarchy.''}

% \subsection{Addressing Peers}

% Every peer in the IPFS network is identified by its \texttt{PeerID}, which is the cryptographic hash of its public key and is therefore, unique to that peer. As a result, when establishing a secure channel, the hash is used to verify that the public key used to secure the channel is the same to the one used to identify the peer (\ie the PeerID). The PeerID makes use of the \textit{Multihash} format discussed earlier and is adding a small preamble/header to specify the hashing algorithm used to produce the PeerID. The format of a PeerID is similar to the one shown in Fig.~\ref{fig:names}.

% The flexible and modular format of \textit{Multiaddresses} allows for the construction of composable addresses that include both network protocol identifiers (location Multiaddresses) and peer identifiers (identity Multiaddresses). 
% For example, libp2p's registered\footnote{\url{https://github.com/multiformats/multiaddr/blob/master/protocols.csv}} protocol id ``\texttt{/p2p/}" can be combined with:
% \begin{enumerate}
%     \item the Multihash of the PeerID (\texttt{\textcolor{gray}{/p2p/}QmZyWQ14..}), which uniquely identifies the peer within the realm of an application that uses libp2p.
%     \item the network location of a peer in the form of its location mMltiaddress: \texttt{/ip4/1.2.3.4/tcp/3333\textcolor{gray}{/p2p/QmZyWQ14..}}.
% \end{enumerate}


% \begin{figure}[h]
% \begin{centering}
% \small
% $
% \underbrace{\overbrace{\hbox{\texttt{/ip4/1.2.3.4/}}}^{\parbox{2cm}{\centering Network Layer}}}_{\parbox{3.0cm}{Protocol \& Address}} 
% \oplus \ \ \underbrace{\overbrace{\hbox{\texttt{tcp/3333/}}}^{\parbox{1.8cm}{\centering Transport Layer}}}_{\hbox{Protocol \& Port}}\
% \oplus \ \ \underbrace{\overbrace{\hbox{\texttt{p2p/QmZyWQ14...}}}^{\parbox{2cm}{\centering P2P Overlay}}}_{\hbox{PeerID}}\ 
% $
% \caption{Multiaddress Structure \& Examples}
% \label{fig:names}
% \end{centering}
% \end{figure}




% \subsection{IPFS Architecture Components}
% % or IPFS Protocol Stack 

% [TEXT TO BE EXCLUDED.]

% The IPFS Architecture is composed of a collection of subsystems each of which can be used independently of IPFS, but together form the foundation for this distributed, content-addressable, P2P storage and delivery network.

% \begin{itemize}
% \item \textbf{libp2p} is a modular network-layer library for P2P networks. In libp2p, peers are identified by the hash of their public key. The library includes all the essential protocols to discover and connect peers, that is, from peer-discovery to peer routing using a DHT and a pubsub protocol (among others), NAT-traversal and provision for several different transports that are easy to integrate. 
% \item The \textbf{InterPlanetary Linked Data (IPLD)} layer is a naming and data management layer used by IPFS. IPLD builds on the concept of ``Merkle-DAGs", that is, Merkle-Trees out of Directed Acyclic Graphs. Every file added into the IPFS system is converted into a Merkle-DAG, locally on the device that adds the file. Each node of the DAG has its own content address, which is the result of hashing of the content itself. Once converted, every node within the DAG is compatible with any data structure that wishes to make use of them or include them as nodes in their own DAG.
% \item \textbf{Multiformats} is a set of formatting rules with specific structure that is used to declare the set of protocols used in a P2P session. In other words, Multiformats is a data representation scheme that adds \textit{self-describing} attributes to the data it formats.
% \end{itemize}

\yiannis{At some point we should make a note of the fact that we're mainly focusing on go-ipfs (and dependencies). We leave out js-ipfs etc, which provide different functionality and is a content routing subsystem of its own that does not use the DHT and pubsub. We could have a subsection here to talk about the different implementations and note which ones we're focusing on?}


% \subsection{Notes on Terminology}

% \yiannis{Might be a good idea to exclude this part. Not sure it adds much.}

% IPFS is commonly being referred to as an Architecture, a Network, or a Protocol (suite). For the purposes of this paper, we refer to IPFS as the Architecture, but provide some more general clarifications on terminology.

% %Due to the wide adoption of IPFS from early on in its lifetime, as well as the changes that the architecture had been undergoing in the meantime, several important terms have been used in wrong contexts. Here we provide some clarifications with regard to the terminology, which we hope to resonate with the community from now on.

% \begin{itemize}
%     \item \textbf{IPFS Architecture:} a distributed, peer-to-peer, content-addressable storage and delivery network. The IPFS Architecture is composed of a suite of protocols that includes both network- and application-layer protocols.

%     \item \textbf{IPFS Main/Public Network:} There is a public, operational IPFS network, but the IPFS protocol stack can be used independently of the main network. The same set of protocols can be used to build a private network that does not need to interact or connect to the main/public network.
%     \item \textbf{IPFS Protocol:} a hypermedia protocol that defines, chunking and naming of content (with help from independent projects such as IPLD and Multiformats). IPFS is responsible for the Content Discovery process, that is for resolving a content identifier (CID) to a peer identifier (PeerID).
%     \item \textbf{libp2p:} a networking library that defines the PeerID and peers' multiaddresses and has mechanisms to establish stream multiplexers, secure channels and do NAT traversal. libp2p does Peer Discovery and Peer routing. There is nothing in libp2p that pre-requisites, uses or outputs content addressing as a fundamental network primitive.
% \end{itemize}



% \subsection{Mapping Content to Peers}\label{libp2p-dht}

% The main task of IPFS is to map content identifiers to peers. 
% %%% IC: DHT now covered in architecture revisit
% For this, IPFS uses a Distributed Hash Table (DHT), provided by the libp2p \hl{[]} library, to bring together CIDs and PeerIDs in a common hash space and enable content and peer discovery and resolution in a decentralized fashion. In particular, the DHT is used to store Provider Records.

% IPFS's DHT is primarily based on Kademlia \cite{maymounkov2002kademlia} with the XOR-distance used as the distance metric between two nodes.

% Nodes in the libp2p DHT use 256-bit keys (as opposed to 160-bit keys used in original Kademlia) and maintain $i=256$ buckets of $k-$nodes each (where $k=20$) to split the hash space. The hash space split is used to store provider records, as discussed in Section~\ref{sec:provider-records}. A provider record is stored to the 20 nodes that are closest in terms of XOR distance from the hash of the content being added to the network. 
% %%%

% \gareth{Add back of the envelope calc for 20 then revisit in evaluation}

% For any lookup, a node initiates $a=3$ concurrent requests from the bucket closest to the requested ID. In contrast to the original Kademlia specification \hl{[link to paper]}, which uses UDP for message transmission, the libp2p DHT is using reliable transports (\ie TCP, or QUIC). \hl{add what this means and why it's done if space permits.}
%This is the \texttt{FIND\_NODE(ID)} message to which each of the $a$ nodes reply with the address of the target node ID, or with the hash of the node(s) closest to the requested node ID that they know of. The procedure repeats until the request reaches the target ID.

%%IC: moved to architecture
% As a measure to improve the scalability and locality properties of Kademlia DHT, the libp2p DHT borrows \textit{sloppy hashing} (from \hl{[]}). According to sloppy hashing, keys for popular content can be stored in intermediate nodes from the requestor to the target ID, breaking somewhat the consistency of traditional DHTs. The rationale is to avoid overloading with requests nodes that hold popular keys.

\subsection{Retrieving Content from IPFS}\label{content-routing}

% Retrieving content from IPFS is composed of three procedures: 
% \one~Content Discovery;
% \two~Peer Discovery;
% and 
% \three~Peer Routing. In this Section, we describe each one of these procedures in turn, but we start by giving some more details about IPFS's Distributed Hash Table (DHT), which serves as the most widely used resolution system of IPFS and the one of interest in this study.\footnote{It is important to highlight that the DHT is only one of the content routing subsystems provided by libp2p with alternatives, such as mDNS, js-ipfs, \hl{++}, being available and operational.}


% Peer Discovery \& Peer Routing are part of libp2p. Both Content \& Peer Discovery utilise libp2p's Distributed Hash Table (DHT). It is important to highlight that the DHT is only one of the content routing subsystems provided by libp2p with alternatives, such as mDNS, js-ipfs, \hl{++}, being available and operational. There are several libp2p protocols involved in the content resolution and delivery, such as techniques for NAT-Traversal and Stream Multiplexing \hl{[link to repos]}. Due to space limitations, here we will only refer to those components of libp2p that are essential for content resolution and delivery and provide links to the rest, where appropriate.



We now proceed to describe the three steps involved in content retrieval, namely, \one~Content Discovery;
\two~Peer Discovery;
and 
\three~Peer Routing.

\pb{Content Discovery.} The libp2p DHT implements \textit{multi-round iterative lookups} in order to resolve a CID to a peer's multiadddress. When peer $x$ issues a request for CID $y$, the request is forwarded to $a=3$ \hl{[]} nodes whose PeerIDs are closest to $y$ in peer $x$'s routing table. The peers receiving those requests reply with the requested content object, if they have it. If they do not have the requested content item, they reply with either the provider record that points to the PeerID that holds the requested item together with the peer's multiaddress (if they have it), or the peers it knows of whose PeerID is closer to $y$. The process continues until the node is returned with the PeerID that has previously declared to hold a copy of the requested CID through a published provider record.

\pb{Peer Discovery.} After the content discovery phase, the requesting peer knows the PeerID of the content (CID) it is looking for, but in many cases the requesting peer still does not know the multiaddress of the peer it needs to connect to. As mentioned earlier, PeerIDs in libp2p are multihashes and therefore, they have to be resolved to a physical network address. This procedure is called \emph{Peer Discovery}. If peer discovery has not taken place together with content discovery (\ie when the multiaddress is returned together with the PeerID), it is carried out by ``walking" the DHT for a second time.

\pb{Peer Routing.} Once the PeerID is resolved through the second DHT walk, the requesting peer has obtained the multiaddress of the peer that appears to have the content. It therefore, uses this multiaddress to connect to and fetch the content.


\pb{Bitswap: The Block Exchange Protocol}
\label{sec:bitswap}

Once a set of storage locations have been identified, the next step is for the client to download the segments. This is done using Bitswap, which is a simple chunk exchange protocol. 

% \gareth{Another quick pointer: this above paragraph doesn't actually start by explaining what Bitswap does. I've rewritten it now, but I've noticed this a few times. We start of a subsection introducing a new concept of compeonent. But we forget to actually explain what the component does or the role it plays in IPFS.}

Due to its simple design, Bitswap can, in certain cases, complete content and peer discovery faster than the DHT.
For this reason, Bitswap makes a content discovery attempt before the DHT actually kicks in.
Bitswap utilises the list of peers that a specific node is connected to.\footnote{IFPS nodes keep a long list of connected peers (up to \hl{900}), which is the list of all the peers that a node has ever seen, or interacted with. Apart from peers that belong to the node's DHT routing table, this list includes peers that do not fall into any of the peer's DHT routing table entries (\ie k-buckets).} 

When a client wants to retrieve a file from IPFS, it explicitly asks \textit{all of those connected peers} for the items it wants - this is the \textit{wantlist} of the peer in the Bitswap protocol. Requests are sent out using an \texttt{IWANT-HAVE} message which prompts those peers that have the block to reply with a corresponding \texttt{IHAVE} message. The requesting peer then responds with an \texttt{IWANT-BLOCK} message. Receipt of the requested block terminates the exchange. The full details of the Bitswap protocol design as well as a number of proposed optimizations can be found in \hl{[link to paper]}.

% There are a number of optimisations done to the above procedure in order to speed up content retrieval with Bitswap.

% \begin{enumerate}
% \item \textit{Peer Choice:} Choosing which peer to ask for the \texttt{IWANT-BLOCK} message is done probabilistically - \hl{add based on what?}
% \item \textit{Bitswap Sessions:} It is very likely that peers who have one block of an object have the rest of the blocks too. Therefore, Bitswap groups those peers who have replied with an \texttt{IHAVE} message into one \textit{session} and is asking those peers for the subsequent blocks of the content item only.
% \item \textit{Small Blocks:} In case of very small blocks \hl{(in the order of [size?])}, peers that receive an \texttt{IWANT-HAVE} message reply with the block itself, rather than an \texttt{IHAVE} message. This is to avoid an extra RTT.
% \end{enumerate}


% \subsection{Content Discovery \& Routing Summary}

% Summarising, the steps followed to discover content and fetch content in IPFS are as follows:
% \hl{[ideally show in figure too]}
% \begin{enumerate}
% \item Get CID (out of band)
% \item Broadcast the WANTLIST to all of the connected peers.
% \item If no IWANT-HAVE message is received proceed to DHT search.
% \item Walk the DHT to resolve CID to PeerID. The DHT will return the multiaddress in addition to the PeerID, if it has it.
% \item As a fallback in case the multiaddress is not returned together with the PeerID from the previous step: Walk the DHT again to get the multiaddress of the PeerID
% \item Contact PeerID to ask for content
% \item Fetch content using Bitswap by sending the WANTLIST to the PeerID and cache a copy
% \item Serve local copy upon subsequent request
% \end{enumerate}

% \gareth{I would remove this above list.}
% \yiannis{I still think it's valuable to show the sequence, but, as discussed, better do it in a figure and include upfront. Commenting out the subsection for now.}

==> archive/4.extensions.tex <==
\section{Extensions}

There are a few extensions or enhancements to the main architecture described so far. These extensions target hassle-free access to content hosted on IPFS through IPFS Gateways (see Section~\ref{ipfs-gateways}) and content discovery speed up through a special type of node, called Hydra Boosters, which store all of the provider records in the IPFS Network (Section~\ref{hydra-boosters}).

\gareth{Do we want to present these as 'extensions'? Could we not present them as a core part of the system?}

\subsection{Hydra Boosters}
\label{hydra-boosters}

\yiannis{TODO: Add description.}


\subsection{IPFS Gateways}
\label{ipfs-gateways}

As the name suggests, an IPFS Gateway is an entry point (or a bridge) for normal browsers to the IPFS network. It enables users that do not run any IPFS software on their machine to access content hosted in the IPFS network. The Gateway is facing: i) the IPFS network from the one side acting as a DHT Server node and, ii) client browsers from the other side, acting as a web server.

Any user or institution can run a Public IPFS Gateway and operation of gateways does not need to be authenticated beforehand by any centralized authority. Public IPFS Gateways, however, need to have a public IP address, \ie not be behind a NAT.

Assuming a user wants to access content with CID \texttt{Qm123xyz..} through a gateway with address \texttt{https://bobs-ipfs-gateway.io/}, they would have to lookup the following URL through their browser:

\texttt{https://bobs-ipfs-gateway.io/ipfs/QmZyWQ14..}

\begin{figure}[h]
\begin{centering}
\small
$
\underbrace{\overbrace{\hbox{\texttt{https://bobs-ipfs-gateway.io/}}}^{\parbox{2cm}{\centering URL}}}_{\parbox{3.0cm}{Gateway Address}} 
\oplus \ \ \underbrace{\overbrace{\hbox{\texttt{ip[f|n]s}}}^{\parbox{1.8cm}{\centering IPFS or IPNS}}}_{\hbox{Protocol Used}}\
\oplus \ \ \underbrace{\overbrace{\hbox{\texttt{/QmZyWQ14}}}^{\parbox{2cm}{\centering CID}}}_{\hbox{Identifier}}\ 
$
\caption{Full URL address to retrieve content through a Gateway}
\label{fig:names}
\end{centering}
\end{figure}

The first part of the URL points the request to the specific gateway (using legacy DNS infrastructure). When the gateway receives the request, it strips off the first part and looks up the CID in the IPFS network, as described earlier in this section. When the gateway receives the content from the IPFS network, it sends it back to the user's browser.



% \subsection{IPFS Cluster}
% \label{ipfs-cluster}

% IPFS Cluster is an application of the IFPS Protocol Stack, which can be used in a private environment. The cluster consists of peers that form a private swarm. Cluster peers use the same protocols as any other IPFS node (\ie DHT, BitSwap, naming conventions and multiaddresses), but they are isolated and not connected to the public IPFS network (or any other private cluster). Cluster peers can be collocated within the same LAN, or be distributed in different WANs. 

% In contrast to the main IPFS network, whose purpose is to serve as a distributed storage and retrieval network without (proactive) replication features, \textit{the purpose of IPFS Cluster is to keep a synchronised view of all entries in every cluster peer}. In order to coordinate concurrent updates from different peers in the swarm and make sure state is synchronised (or shared) between them (\ie guarantee Strong Eventual Consistency), IPFS Cluster makes use of consensus algorithms. There are currently two consensus algorithms implemented as part of IPFS Cluster, one of which needs to be selected in the cluster setup process with the choice depending on the characteristics of the application running on top (\eg expected rate of node churn):
% \begin{enumerate}
%     \item \textbf{Raft Consensus:} This is the traditional Raft consensus algorithm \hl{[]}, which assumes stable connectivity of peers and broadcasts updates to all cluster peers.
%     \item \textbf{Merkle-CRDTs:} This is a newly-proposed \hl{[]} consensus algorithm which combines properties of Conflict-free Replicated Data Types (CRDTs) with append-only, immutable Merkle Directed Acyclic Graph structures. The resulting algorithm provides strong eventual consistency and the potential to greatly simplify the design and implementation of convergent data types in systems with weak messaging layer guarantees and a very large number of replicas.
% \end{enumerate}


==> archive/5.methodology.tex <==
\section{Evaluation Data}
\label{sec:methodology}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{plots/plot_crawl_network_size_gateway_load.pdf}
    \caption{a) Total number of crawled peers over time and their fraction of dialable and undialable peers. The graph shows a one-day periodicity. The graph shows several events and measurement time periods which help to assess and judge our measurement results in later sections. b) Request count of a single Gateway on 2022-01-02.}
    \label{fig:plot_crawl_network_size_gateway_load}
\end{figure*}

At this point we have covered IPFS' fundamental building blocks, the content lifecycle in the network, and design decision made along the way. Now we want to evaluate the success of the IPFS network.
However, due to its decentralized nature, it is not possible for us to record activities across all IPFS nodes, as the majority are run by independent node operator.
Hence, to evaluate IPFS, we rely on four datasets comprising a mix of active and passive measurements, alongside gateway log collection.
We use these four datasets to evaluate the network deployment, content routing performance, and protocol overhead that follow in Sections~\ref{sec:deployment} and \ref{sec:evaluation}. As these datasets have been gathered over time, Figure \ref{fig:plot_crawl_network_size_gateway_load}a presents a timeseries overview of our measurement periods. This figure is explained further in the subsequent sections. 

\subsection{Peer Data}
\label{sec:methodology_network_crawls}

%A major performance indicator for an unstructured peer-to-peer network is participant churn, meaning how long do peers stay in the network after joining before going offline again. Network-wide parameters that cover the number of record replication and request concurrency rely on an accurate understanding of this dynamic. Further, we want to understand the geographical and autonomous system distribution of peers, capture shifts over time and derive public cloud provider coverage.

Our first dataset covers information about peers running the DHT. As there is no central repository of such information, we employ an active measurement methodology to gather this data. 
Specifically, we implement a crawler\footnote{\url{https://github.com/REDACTED}} to gather a comprehensive list of peers.
Figure \ref{fig:plot_crawl_network_size_gateway_load} presents the number of peers observed each day.
We make our crawl data available on IPFS with the CID\footnote{ \texttt{bafybeigkawbwjxa325rhul5vodzxb5uof73neszqe6477nilzziw5k5oj4}}.

%It has an emphasis on continuous node monitoring to allow for high accuracy session length measurements and highly normalized RDBMS-backed data persistence that on the one hand yields a low data footprint and on the other hand allows near-arbitrary retrospective analyses.

% The \hl{first} active network measurement method constitutes a newly developed DHT crawler\footnote{\url{https://github.com/REDACTED}} with an emphasis on continuous node monitoring to allow for high accuracy session length measurements and highly normalized RDBMS-backed data persistence that on the one hand yields a low data footprint and on the other hand allows near-arbitrary retrospective analyses. Henningsen et al. \cite{HenningsenFRS20} previously presented a network crawler with a similar feature set. However, the crawler in \cite{HenningsenFRS20} lacks capabilities in the areas mentioned above. Further, the clear distinction of DHT client and server nodes introduced in \texttt{go-ipfs v0.5.0} vastly changed the network topology landscape and justifies revisiting previous results.

The crawler recursively asks peers in the network for all entries in their $k$-buckets starting from the six well-known default IPFS bootstrap peers until it finds no new entries. The procedure that yields the list of all $k$-bucket peers resembles previous work on IPFS crawlers like \cite{HenningsenFRS20}.
% After connecting to a remote peer, the crawler constructs its routing table based on their peer ID.
% Then, it generates random peer IDs with common prefix lengths (CPL) that fall within each $k$-bucket of the just constructed routing table.
% Lastly, the crawler asks the remote peer for closer peers for each generated CPL peer ID. This is done by performing concurrent \texttt{FIND\_NODE} RPCs for all CPLs.
% This approach will effectively yield a list of all peer IDs that a peer has in its routing table. The process repeats for all returned peers until the crawler finds no new peers.

We have run the crawler from Germany every 30 minutes. We started our measurements on 2021-07-09 and upgraded it on the 2021-09-24 to allow the association of single peers with their Multiaddresses, agent version, supported protocols, and dial, handshake and crawl duration.
In total, we have performed over \num{9500} network crawls.
We geolocate each observed IP address using the GeoLite2 Country Database; and we map IP addresses to ASNs using the GeoLite2 ASN Database. Further, we associate each ASN with its CAIDA AS Rank. 

%Each crawl took \SI{5.3\pm 1.1}{\minute} assuming a normal distribution of crawl times.

To identify peer uptime, we revisit all previously discovered and online peers periodically and track their session lengths along the above parameters.
Due to the scale, we adapt the revisit frequency based on how often we observe a peer. 
Specifically, we select an interval of half of the observed uptime starting at a minimum of 30 seconds and a maximum of 15 minutes.
We base this procedure on the assumption that it is more likely for peers to stay online if we observed them to have been online for a longer time period. 



%\subsubsection{General}

%The crawler is running on a Hetzner Ubuntu 20.04.3 CPX31 virtual machine in Germany. We started our network measurements on 2021-07-09 and increased the data collection granularity on the 2021-09-24 to allow the association of single peers with their agent version, Multiaddresses, and supported protocols. For all graphs below, if not noted otherwise, we consider the measurement period from the 2021-10-01 until 2021-11-01 as depicted with ``Detailed Analysis'' in Figure \ref{fig:crawl_network_size_agents_combined}. We started the data analysis in December 2021 and wanted to analyse one full month of uninterrupted data collection.



%obtain autonomous system ranking information from ``AS Rank'' by querying their API \texttt{v2.1} on 2022-01-18\footnote{\url{https://api.asrank.caida.org/v2/docs}}.

% \gareth{There is a lot of text above that doesn't really convey much information. It would be better to be concise and clear. We can state the purpose of the data collection, and then describe it step by step. Some of the stuff about RAM, granularity, tracking metrics etc is probably a bit too fuzzy to convey any real meaning}

%\subsubsection{Crawl Procedure}
% \gareth{I would condense the above and make this part the main body of the section.}

%\subsubsection{Dataset}

%Our IPFS network crawls started at 2021-07-07 and the data set contains information until 2022-01-22 as two different postgres dumps divided at 2021-11-24. However, neither does contain the original Multiaddresses, nor IP-addresses for privacy reasons. We call the connection attempt to a remote peer either through a crawl or during monitoring a ``visit" which can either succeed or fail. In the former case the crawler tracks information timestamps, dial duration, Multistream protocol negotiation duration, crawl duration, set of supported protocols, agent version, set of Multiaddresses plus their encapsulated IP addresses and session length information. In the latter case of an error it tracks the reason and Multiaddress information. Starting from 2021-11-26 we started to persist the $k$-bucket entries of each peer we found during network crawls. This allows granular network topology analyses.

\subsection{IPFS Gateway Usage Data}
\label{sec:methodology_gateways}

An IPFS Gateway\footnote{Any user or institution can run a Public IPFS Gateway. Operation of gateways does not need to be authenticated beforehand by any centralized authority. Public IPFS Gateways, however, need to have a public IP address.} is, as the name suggests, an entry point for Web browsers to the IPFS network. It enables users that do not run any IPFS software on their machine to access content hosted in the IPFS network. On the one side, Gateways face the IPFS network acting as a DHT server node, and on the other side, they face client browsers acting as a web server. Hence, they are able to map location-based HTTP requests to the content-addressed IPFS network, acting as a bridge.

%An important aspect to ease the transition to a decentralized Web is to provide bridges between both worlds. Public . By using public gateways users lose automatic data integrity checks that IPFS provides natively. Public gateways can be hosted by any party voluntarily. 

Our second dataset covers all the requests taken from a public IPFS Gateway run by us
% Protocol Labs (\texttt{ipfs.io}) 
giving vantage into large-scale usage patterns of IPFS. The dataset covers one day of access in January 2022, with 1.22\,M access entries from 7.1\,M requests. Each access log entry maps to a single user request and response meta data to the gateway. The data comprises of timestamp, user agent, HTTP referrer, city and response sizes with the information of responses being cached or not on the server. The city information is identified using Maxmind by mapping the anonymized IP addresses to their geolocation. Further, for each request entry, we generate a user identifier by computing the hash of {anonymized IP address, device}. Overall we find 101\,k users accessing 274\,k CIDs via the gateway. Figure~\ref{fig:plot_crawl_network_size_gateway_load}b shows the request load binned every five minutes at the gateway based on the timezone of the user requesting and of the gateway serving the content. A median of 22.4GB is sent every 5 minutes. As expected, the majority are http \texttt{GET} requests (\SI{98.22}{\percent}) and \SI{1.56}{\percent} are \texttt{POST} requests.  To avoid requests made by the administrators to configure the gateway, we proceed our analysis with the \texttt{GET} requests. We make the access logs available on IPFS with the CID\footnote{ \texttt{\hl{PRIVACY PRESERVING CID OF LOGS}}}.


\subsection{Performance Data}
\label{sec:methodology_dht_lookups}

Our third dataset focuses on benchmarking lookup performance. 
We use six virtual machines in six different regions using AWS. Namely, the \texttt{t2.small} machines run in \texttt{me\_south\_1} (Bahrain), \texttt{ap\_southeast\_2} (Sydney), \texttt{af\_south\_1} (Cape Town), \texttt{us\_west\_1} (N. California), \texttt{eu\_central\_1} (Frankfurt) and \texttt{sa\_east\_1} (S\~ao Paulo). 
On each machine we install and start a modified \texttt{go-ipfs v0.10.0} instance. The modifications consist of additional log messages to gather information about peer interactions. 

%Next to each IPFS instance we install an agent that can control the instance and in turn accepts commands by a central controller. The central controller instructs the IPFS instances, via the agents, to publish or retrieve carefully crafted CIDs into/from the network.

We then use these instances to publish and retrieve IPFS objects. 
Upon each iteration, a single node announces a new object to the network (size $0.5\,\mathrm{MB}$).
Following this, all other nodes retrieve the object.
This involves looking up the provider record, connecting to the provider and then downloading the object. As soon as all remaining nodes have completed this process, they disconnect. 
Table \ref{tab:dht_pvd_ret_counts} lists the number of publications and retrievals we have performed from each region. The data is published on IPFS with the CID\footnote{
\texttt{bafybeid7ilj4k4rq27lg45nceq4akdpetav6bcujgiym6vch5ml24tk2t4}}.


%The controller starts with generating $0.5\,\mathrm{MB}$ of random data. It then transfers this data to the first controlled IPFS instance and instructs it to announce to the IPFS network that it is in possession of this data. This step resembles the content publication process. As soon as this step has finished the controller instructs all remaining controlled IPFS instances to retrieve the CID of the random data.

%This step involves finding the provider record, connecting to the provider (first controlled IPFS node) and then fetching the $0.5\,\mathrm{MB}$ of random data. As soon as all remaining IPFS instances have completed this process the controller instructs them to disconnect from the provider. This last step is done so that we avoid retrieving content through Bitswap during the next experiment, since peers would remain directly connected. In other words, this would test the performance of Bitswap and not the DHT lookup process.

%\subsubsection{Dataset}

\begin{table}[]
    \centering
    \footnotesize
    \caption{Number of publication and retrieval operations from each AWS region.}
    \label{tab:dht_pvd_ret_counts}
    \vspace{-0.3cm}
    \begin{tabular}{lrr}
        \hline\hline
        AWS Region                & Publications & Retrievals \\ \hline
        \texttt{af\_south\_1}     & $547$ & $2,047$ \\
        \texttt{ap\_southeast\_2} & $547$ & $2,630$ \\
        \texttt{eu\_central\_1}   & $547$ & $2,708$ \\
        \texttt{me\_south\_1}     & $547$ & $2,112$ \\
        \texttt{sa\_east\_1}      & $546$ & $2,363$ \\
        \texttt{us\_west\_1}      & $547$ & $2,704$ \\ \hline
        \textbf{Total}            & $3,281$ & $14,564$ \\
        \hline\hline
    \end{tabular}
    \vspace{-0.3cm}
\end{table}


\subsection{Open Source Data}
\label{sec:methodology_public_domain}

\newcommand\shaSpecs{bab189ee}
\newcommand\shaGoIPFS{6fb73c45}
\newcommand\shaJsIPFS{c083645e}
\newcommand\shaRustIPFS{ad3ab49b}

Peers in the IPFS network follow a set of technical protocol specifications\footnote{SHA1: \texttt{\shaSpecs} -- \url{https://github.com/ipfs/specs}} of which there exist one reference implementation written in Go and two implementations in alpha state written in JavaScript and Rust. The results shown below were gathered directly from their respective git repositories go-ipfs\footnote{SHA1: \texttt{\shaGoIPFS} -- \url{https://github.com/ipfs/go-ipfs}}, js-ipfs\footnote{SHA1: \texttt{\shaJsIPFS} -- \url{https://github.com/ipfs/js-ipfs}} and rust-ipfs\footnote{SHA1: \texttt{\shaRustIPFS} -- \url{https://github.com/rs-ipfs/rust-ipfs}} and were collected on the 9th of December 2021.


==> archive/6.deployment.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Deployment Scale}
\label{sec:deployment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{plots/crawl_geo_map_peers.pdf} 
    \caption{Geographical distribution of peers.}
    \label{fig:crawl_geo_map_peers}
\end{figure}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{plots/crawl_geo_combined.pdf} 
    \caption{a) Geographical distribution of peers that were reachable for \SI{>90}{\percent} of the measurement period. Note the \textperthousand~unit on the y-axis. b) Geographical distribution of peers that were always offline and not reachable at all during the measurement period. c) Geographical distribution of physical machines as identified by their unique IP addresses categorized in a set of reachable and unreachable nodes. d) IP address AS distribution.}
    \label{fig:crawl_geo_combined}
\end{figure*}

\noindent In this section, we make use of our datasets and present how peers, physical machines and Gateway users are geographically distributed. Further, we evaluate the autonomous system coverage to spot potential cloud provider centralisation. At the end of this Section, we highlight the key takeaways. Unless noted otherwise, we limit our evaluation to the shaded area labeled ``Detailed analysis'' in Figure~\ref{fig:plot_crawl_network_size_gateway_load}a.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Geographical distribution}
\label{sec:geographical_distribution}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We first turn to our Peer Dataset. In total, we discover \num{198964} peers with \num{1998825} Multiaddresses in the DHT which cover \num{464303} IP addresses. Since a single physical host can register itself with a number of peer identities in the DHT, we analyse the geographical distribution from two different perspectives: We analyse \one~The geographical distribution of peer identities; and \two~The geographical distribution of physical hosts as identified by their IP addresses.

% The decentralized nature of IPFS operations, means that we also discover a wide spectrum of software versions being operated. 
% We observe \num{278} unique agent versions. Figure~\ref{fig:crawl_network_size_agents_combined}b shows the distribution of the most prominent ones. Note, the graph omits older \texttt{go-ipfs} and rare agent versions for clarity as they only represent a small fraction of the total number of peers. The \texttt{storm} and \texttt{ioi} user agents correspond to nodes that use the IPFS overlay network but are not affiliated with the IPFS project.

%An indicator for a healthy, peer-to-peer network is the willingness of participants to upgrade their clients so that the network as a whole can benefit from new capabilities. We learn from the graph that participants indeed upgrade their clients, and only a fraction of peers join the network with clients older than a year. Further, while we cover churn of \texttt{storm} and \texttt{ioi} agents below in Section \ref{sec:churn}, their significant share justify a more targeted analysis which is out of scope of this paper.

% \texttt{storm} nodes are related to a botnet where the node operators may not even know about its existence \hl{cite something about the storm botnet} and \texttt{ioi} user agents

% In the recent history of IPFS a significant network upgrade constituted the \texttt{go-ipfs v0.5.0} release\footnote{\url{https://blog.ipfs.io/2020-04-28-go-ipfs-0-5-0/}} (April 2020).

% Figure~\ref{fig:crawl_geo_map_peers} shows the geographical distribution

% \subsection{Agent Version Distribution}

% An indicator for a healthy, peer-to-peer network is the willingness of participants to upgrade their clients, so that the network as whole can benefit from new capabilities. In the recent history of IPFS a significant network upgrade constituted the \texttt{go-ipfs v0.5.0} release\footnote{\url{https://blog.ipfs.io/2020-04-28-go-ipfs-0-5-0/}} (April 2020). It introduced the DHT client mode and vastly decreased the number of unreachable peers in the DHT. Inaccessible peers behind NATs would not join the DHT as a server node. As of this writing the latest \texttt{go-ipfs} release is version \texttt{0.11.0} from 2021-12-09.

% Figure~\ref{fig:crawl_network_size_agents_combined}b shows the agent version distribution of the IPFS network for the complete measurement period. We see the uptake of the most recent go-ipfs releases on 2021-10-01 and 2021-12-09. However, the majority of network participants still run \texttt{go-ipfs v0.8.0} until the network saw a significant increase in size recently. \texttt{go-ipfs v0.9.0} now dominates the network, which is still two releases behind. Similarly, \texttt{go-ipfs v0.7.0} increased its dominance in the network, as well. The graph omits older \texttt{go-ipfs} and rare agent versions for clarity as they only represent a fraction of the total number of network participants.

% The \texttt{storm} and \texttt{ioi} user agents on the other hand correspond to nodes that make use of the IPFS overlay network but are not affiliated with the IPFS project. \texttt{storm} nodes are related to a botnet where the node operators may not even know about its existence \hl{cite something about the storm botnet}. The daily periodicity may hint at a usage pattern that correlates with daily start-up and shutdown of personal computers in a particular time zone.

% \texttt{ioi} nodes also reveal a one-day...

% \gareth{The above is very verbose, but doesn't really reveal anything that important. It might be worthwhile condensing this, or even integrating it into the Overview subsection previously? COuld just point to it and have a single paragraph summarising the observations?}



% We next inspect the uptake of IPFS across the world using our GeoIP mappings for the \num{464303} IP addresses extracted from the DHT. Note, peers can be reached via a proxying peer that relays the traffic in case it is not publicly reachable themselves. We exclude those Multiaddresses as it would skew the geographical distribution towards the locations where relaying peers reside. 


% Total: 198,964
% No multi_address_set_id: 2,946
% Associated Peers: 196,018
% Multiple Countries: 18,846

\pb{Geographical Distribution of Peers.}
Figure~\ref{fig:crawl_geo_map_peers} shows the geographical distribution of peer identities.
Although we see widespread uptake, we do note a high dependency on certain regions. 
The US and China dominate the share of peers, followed by France, Taiwan, and South Korea.
Multihoming seems commonplace: Around \SI{9.5}{\percent} of all peers advertise Multiaddresses to the network that link to IP addresses which we could associate with multiple countries.\footnote{Note, in Figure~\ref{fig:crawl_geo_map_peers} such peers were counted repeatedly for each country or region they appeared in.}
This effect is particularly evident for peer identities we could associate with France, where 90\% of peers were associated with IP addresses based in other countries. 
\yiannis{Might be worth mentioning what this means in practice, e.g., for the operation of the DHT, any effect on lookup latency observed?}

If we now group the peers by their reliability and reachability we observe in Figure \ref{fig:crawl_geo_combined}a and \ref{fig:crawl_geo_combined}b a different distribution. Highly reliable peers are those that exhibit \SI{>90}{\percent} uptime during the measurement period. 
In total, \num{2747} peers (\SI{1.4}{\percent}) fall into this category. Unreachable peers are those that never responded, of which we find \num{65787} (1/3) in the DHT.
However, an unambiguous country association for the latter is not always possible as some exclusively provide: \one~IP addresses in private CIDR ranges, \two~circuit relay addresses \three~unresolvable DNS Multiaddresses, or were: \four~associated to multiple countries, \five not found in the GeoIP database. The remaining \num{60411} peers still account for \SI{92}{\percent} of all unreachable peers.

Clearly, for the cohort of reliable peers the Chinese dominance decreases but still plays a major role. Nodes from the US and Germany lead this group. The same three countries also lead the cohort of unreachable peers but with a clear Chinese dominance raising questions about the relevance of the ``Great Firewall''.

% While the geographical distribution of IP addresses gives a good idea of possible agglomerations, less represented countries may provide a more reliable service.


% In the following subsections, we cover the geographical distribution of always offline peers and peers that we consider reliable as defined below. The sample sizes that the graphs below are based on are given in Table \ref{tab:deployment_overview} in the respective ``Peer IDs'' and ``IP Addresses'' segments.

% \gareth{I'm not sure it's necessary to breakup the peers into offline vs reliable. Instead, I guess the point is to present the geodistribution. So, you could perhaps start with a map of the peers per country. Then talk about which countries dominate. Then ideally say that the picture is not that simple, because many in certain countries like China are often offline. }

% \num{2946} of them did exclusively provide IP addresses in private CIDR ranges, \num{981} did exclusively provide circuit relay addresses, and four peers provided DNS Multiaddresses that could not be resolved to IP addresses. Out of the remaining \num{61856} peers, \num{1436} were found with multiple IP addresses that we can link to multiple countries and finally, nine were not found in the Maxmind database. The final \num{60411} peers still account for \SI{92}{\percent} of all unreachable peers and Figure \ref{fig:crawl_geo_combined}b shows their geographical distribution.
% Note that the remaining peers may have announced different IP addresses to the IPFS network which were mapped to a single country and hence represent just one data point in this consideration.
% The ``Unmapped'' bar is barely visible as it only accounts for the four unresolvable DNS Multiaddresses and nine IP addresses that were not found in the Maxmind database.

% \subsubsection{Offline Peers}

% We report our findings for Offline Peers in Fig.~\ref{fig:crawl_geo_combined}a. 
% \gareth{I would suggest putting the reliable peers first, and then showing the offline peers afterwards (to highlight that a cursory glance is not sufficient to understand what is really going on}

% We found $65,787$ peers in the DHT that we were not able to dial at all, which account for roughly $1/3$ of all discovered Peer IDs. Each of them registers itself with multiple Multiaddresses in the DHT. However, $2,946$ of them did exclusively provide IP addresses in private CIDR ranges and $981$ did exclusively provide circuit relay addresses. These were filtered out. Additionally, four peers provided DNS Multiaddresses that could not be resolved to IP addresses. Out of the remaining $61,856$ peers, $1,436$ were found with multiple IP addresses that can be associated with different countries and nine were not found in the Maxmind database, so they were excluded as well. The remaining $60,411$ peers account for $92\,\%$ of all undialable peers and Figure \ref{fig:crawl_geo_combined} shows their geographical distribution. Note that the remaining peers may have announced different IP addresses to the IPFS network which were mapped to a single country and hence represent just one data point in this consideration.

% Is the above sentence clear? I mean:
%   - peer A has multi addresses: /ipv4/1.2.3.4/tcp/1234 and /ipv4/5.6.7.8/tcp/1234
%   - peer A has ip addresses: 1.2.3.4, 5.6.7.8
%   - 1.2.3.4 maps to US and 5.6.7.8 maps to US
%   - peer A is mapped to the US although it may be reachable on two different hosts.

% \dennis{What's the take away?}
% \yiannis{I suggest we have a subsection at the end of this section to summarise all the takeaways. I've made a start, but please add.}


\pb{Geographical Distribution of Nodes.}
As opposed to the geographical distribution of peer identities the distribution of physical hosts as identified by their IP addresses gives insights about where the networks' compute power and bandwidth concentrates. In total, we were able to establish a connection to \num{211105} (\SI{54.5}{\percent}) IP addresses at least once while \num{211105} (\SI{45.5}{\percent}) we found to be unreachable. Figure \ref{fig:crawl_geo_combined}c shows their geographical distribution.
% The percentages are relative to the total number IP addresses as opposed to each reachability cohort.

Again, hosts from China dominate the network by a wide margin. However, only $1/3$ of nodes in China were actually reachable for us. This raises questions regarding the role of the ``Great Firewall''. The US, on the other hand, is not as dominant anymore hinting at a usage pattern that favors the creation of many peer identities on fewer hosts. Generally, China, Hong Kong, and Taiwan make up more than half of all reachable nodes concentrating a relevant fraction of compute power and bandwidth in (south-)east Asia. The later Section~\ref{sec:autonomous_system_coverage} about the Autonomous System coverage confirms this observation.


\pb{Geographical Distribution of User Requests.}
We now turn to our IPFS Gateway Usage Data and analyze the geolocation of IP addresses that request content through the Gateway. Figure \ref{fig:gateway_geo_map_requests} shows their geographical distribution.

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{plots/gateway_geo_map_requests.pdf} 
    \caption{Geographical distribution of users requesting content via the Gateway.}
    \label{fig:gateway_geo_map_requests}
\end{figure}

Albeit hosting a significant proportion of nodes, we find more than three-quarters of user requests to the gateway come from the US (50.4\%) and China (31.9\%). This is followed by Hong Kong (6.6\%), Canada (4.6\%) and Japan (1.7\%). 

A closer look into the data also reveals that the majority of this traffic (51.8\%)  is referred by third party websites. Interestingly, 70.6\% of this referred traffic belongs to 72 semi-popular websites (rank 10K-50K) when ranked based on Tranco list\footnote{list collected a day after the log capture at the gateway}~\cite{LePochat2019tranco}. We find a majority of these parent sites are hosted in the US (47.3\%), Iceland (20\%), Canada (12.7\%). Thus, though there are innate implications such as request failures and response delays (explained in section~\ref{sec:overhead}), this shows the global usage of public gateways by both  application and users. 
~\aravindh{not sure whether this bit is interesting/makes sense, but also a manual check of these sites indicate majority of them are video streaming service or NFT-related site. is it worth mentioning delay-tolerant applications or just leave it?}
% We notice a significant number of successful requests (56.51\%) are referred from other websites accounting 58.92\% of total response bytes from the gateway. We use this to understand the source of the traffic and present the top sites in Table~\ref{tab:referrer_domains}. 
% The top website to refer 37.72\% of traffic is video delivery website with 98.1\% of requests originating from China.
% \begin{table}
% \caption{Referrer domains resulting in $>80\%$ of requests to IPFS gateway}
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{lrrl}
% \toprule
% Referrer domain &  Bytes transferred (\%) &  Requests (\%) & Description\\
% \midrule
%          nunuyy.top &       64.02 &       62.82 & video delivery website \\
%             ipfs.io &       2.19 &        7.95 & IPFS homepage\\
%       dandanzan.top &        3.65 &        3.82 & video delivery website\\
%       magiceden.io &       3.61 &        2.89 & NFT marketplace\\
%       hicetnunc.art &        5.26 &        2.31 & NFT marketplace\\
%     %   \textbf{all}  &\textbf{58.92}&\textbf{56.51} &\\
% \midrule
% \bottomrule

% \end{tabular}
% }
% \label{tab:referrer_domains}
% \end{table}

\gareth{I think we spend way too much time discussing the above results. They're quite short, but we have a lot of clarification etc. I've tried to cutdown, but I would probably be in favour of dramatically condensing this to become much more succinct.}



\subsection{Autonomous System Coverage}
\label{sec:autonomous_system_coverage}

\pb{AS Coverage.}
Next, we investigate the autonomous system (AS) coverage of the IPFS deployment. 
In total, we see at least one IPFS node in \num{2715} ASes, roughly \SI{3.7}{\percent} of all currently allocated ASes.
Figure~\ref{fig:crawl_geo_combined}d shows the number of IPFS nodes (identified by unique IP address) per AS on y-axis. 
We bucket ASes based on their CAIDA AS Rank on the x-axis. 
We stack the bar to reflect the geolocation of each IP adress.
For context, Table~\ref{tab:asn_to_name_mapping} lists the top ASes that cover \SI{>50}{\percent} of discovered IP addresses.

%shows the AS continent distribution of all found IP addresses. The x-axis shows the first 10\,k ASes ordered by their rank as defined in Section~\ref{sec:methodology_network_crawls} which cover \SI{94.6}{\percent} of all IP addresses. Each 1\,k ASs are combined to one bar. Further,


\pb{Cloud coverage.} Table~\ref{tab:cloud_provider_coverage} lists the number of nodes that are deployed in centralised cloud infrastructure.
We identify cloud IP space by case-insensitively matching AS names against the given keywords.
% These results are inevitably slightly skewed, as small cloud providers do not reveal their IP address ranges. However, given the dominance of large cloud providers and the percentage difference in market acquisition, we expect the error to be negligible.
We see that a minority of \SI{<1.1}{\percent} of IPFS nodes are hosted in centralised cloud infrastructure. This is an important finding for a decentralized storage and delivery network, such as IPFS, and shows that users put up their own deployments.


\begin{table}[h]
    \footnotesize
    \centering
    \caption{Autonomous systems covering \SI{>50}{\percent} of all found IP addresses.}
    \label{tab:asn_to_name_mapping}
    \vspace{-0.3cm}
    \begin{tabular*}{\linewidth}{rrrl}
        \hline\hline
        Share                & ASN & Rank    & AS Name                                              \\ \hline
        \SI{18.9}{\percent}  & 4134 & 76     & \tiny{CHINANET-BACKBONE No.31,Jin-rong Street, CN}          \\
        \SI{12.8}{\percent}  & 4837 & 160    & \tiny{CHINA169-BACKBONE CHINA UNICOM China169 Back., CN}    \\
        \SI{9.6}{\percent}   & 4760 & 2976   & \tiny{HKTIMS-AP HKT Limited, HK}                            \\
        \SI{6.9}{\percent}   & 26599 & 6797  & \tiny{TELEFONICA BRASIL S.A, BR}                            \\
        \SI{5.3}{\percent}   & 3462 & 340    & \tiny{HINET Data Communication Business Group, TW}          \\
        \hline\hline
    \end{tabular*}
    \vspace{0.3cm}
    \caption{Percentage of nodes hosted on cloud providers based on their AS membership.}
    \label{tab:cloud_provider_coverage}
    \vspace{-0.3cm}
    \begin{tabular*}{\linewidth}{lrrl}
        \hline\hline
        Provider      & IP Addresses & Share    & AS Name Keywords \\ \hline
        Amazon        & \num{1791}   & \SI{0.4}{\percent}  & \texttt{aws|amazon} \\
        Microsoft     & \num{1536}   & \SI{0.3}{\percent}  & \texttt{microsoft|azure|msft} \\
        Digital Ocean & \num{852}    & \SI{0.2}{\percent}  & \texttt{digital\textbackslash s?ocean} \\
        Google        & \num{429}    & \SI{<0.1}{\percent} & \texttt{google|gcp} \\
        Alibaba       & \num{300}    & \SI{<0.1}{\percent} & \texttt{alibaba} \\
        Oracle        & \num{41}     & \SI{<0.1}{\percent} & \texttt{oracle|orcl} \\
        % IBM           & \num{0}      & \SI{0}{\percent}    & \texttt{ibm} \\ \hline
        Other         & \num{459354} & \SI{98.9}{\percent} & \\
        \hline\hline
    \end{tabular*}
    \vspace{-0.3cm}
\end{table}


\subsection{Discussion \& Key Takeaways}

We designed IPFS to be a highly decentralized peer-to-peer network. Although we observe geographical agglomeration in certain regions, we also see IPFS being widely adopted around the globe. Especially important is finding of \SI{<1.1}{\percent} IPFS nodes running in centralized cloud environments. This is a prove for people running nodes on commodity hardware. This, however, may also be a reason for the small number of reliable IPFS nodes. Hence, the findings suggest a high churn rate which we verify in Section~\ref{sec:churn}.

Generally, the previous subsections give us a comprehensive understanding of IPFS' current deployment distribution and user base. We note that China dominates in terms of node presence with a share of \SI{45}{\percent}. At the same time China hosts the vast majority of unreachable nodes/peers. This raises questions regarding the role of the ``Great Firewall''. We plan to collect peer data from within China to be able to assess its influence in greater detail. However, we designed IPFS with the key requirements of resiliency against takedown and censorship in mind. Content should only become unavailable in the scenario of a network split for either side.


% We highlight several key observations:

% \begin{itemize}
%     \item China dominates in terms of IPFS node presence (\hl{include percentage?}).
    
%     \item At the same time by the vast majority of always offline and unreachable nodes are based in China. This raises questions regarding the role of the Great Firewall.
    
%     \item Reliable nodes are a very small minority in the IPFS network, which in turn means that there is high rate of churn (as we verify in the next Section).
    
%     \item Less then \SI{1.1}{\percent} of IPFS nodes are run in centralized cloud environments.
    
%     \item Is there a semi-poular app that builds on top of IPFS? I'm thinking of berty which has its HQ in Paris?

%     \item (Limitation due to parallel dial we can't be sure which IP address was actually reached.)
% \end{itemize}

\gareth{Ideally we could include lessons learnt and/or implications above. Were they any steps taken (within the IPFS design) that tries to deal with the above observations?}

==> archive/7.evaluation.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Evaluation}
\label{sec:evaluation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In this Section, we perform a performance and overhead evaluation of IPFS' two core functions: content publication and content retrieval.




% \subsection{Community}

% \begin{figure*}
%     \centering
%     \includegraphics[width=\textwidth]{plots/github_stats_ipfs.pdf}
%     \caption{Insertions and deletions of lines of code in the go-ipfs, js-ipfs and rust-ipfs repositories as well as the number of changed files over time. \hl{In 2019 development focus shifted from go-ipfs to js-ipfs as can be seen from the number of changed files and the steep increase of insertions/deletions}.}
%     \label{fig:github_stats_ipfs}
% \end{figure*}

% \begin{table}
%     \centering
%     \footnotesize
%     \caption{Git and GitHub statistics for the reference implementation go-ipfs and two alpha implementations js-ipfs and rust-ipfs. Git statistics were collected for the respective commit SHA1s below and GitHub statistics were collected on the 2021-12-08.}
%     \label{tab:git_statistics}
%     \vspace{-0.3cm}
%     \begin{tabular*}{\linewidth}{l@{\extracolsep{\fill}}rrr}
%     \hline\hline
%                      & \textbf{go-ipfs}    & \textbf{js-ipfs}    & \textbf{rust-ipfs}   \\\hline
%     SHA1             & \texttt{\shaGoIPFS} & \texttt{\shaJsIPFS} & \texttt{\shaRustIPFS} \\
%     latest release       & \texttt{0.11.0}  & \texttt{0.60.2}   & \texttt{0.2.1} \\
%     \# commits       & $12.8\,\mathrm{k}$  & $6.3\,\mathrm{k}$   & $1.8\,\mathrm{k}$ \\
%     \# loc\footnotemark           & $35.7\,\mathrm{k}$ & $58.8\,\mathrm{k}$ & $20.8\,\mathrm{k}$  \\
%     \# stars         & $12.4\,\mathrm{k}$ & $6.1\,\mathrm{k}$ & $928$\\
%     \# forks         & $2.4\,\mathrm{k}$ & $1.2\,\mathrm{k}$ & $106$ \\
%     \# releases\footnotemark      & $34$ & $721$ & $3$ \\
%     \# contributors  & $299$ & $202$ & $21$ \\
%     \hline\hline
%     \end{tabular*}
% \end{table}
% \footnotetext{lines of code (loc) as reported by \texttt{cloc} \cite{danialcloc21} while only considering the main language for each repository.}
% \footnotetext{js-ipfs includes releases of the \texttt{ipfs} node module and 18 internal packages it depends on.}

% As an open and community-driven effort, we first seek to explore how involved the community is in the development of IPFS.
% We first inspect the breadth of contributors to the IPFS codebase, before inspecting IPFS's deployment footprint.

% A major goal of the decentralised web is to democratise the control, ownership and development of its associated systems and protocols. Thus, a key evaluative metric of our success, is the uptake by the wider development community. To this end, we extract all commit logs from the mainline Git repositories hosted on GitHub.
% % Here, we seek to understand the scale and distribution of the IPFS development community. 
% Table \ref{tab:git_statistics} shows statistics that \hl{++}

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{plots/git_contribution_cdf.pdf}
%     \caption{Git commit authors as a cumulative distribution function for the three major IPFS implementations. The numbers in the legend show the total number of de-duplicated authors for each IPFS implementation.}
%     \label{fig:git_contribution_cdf}
% \end{figure}

% Figure \ref{fig:git_contribution_cdf} shows the commit author count as a cumulative distribution function of the number of commit each author has contributed. The data was obtained via running \texttt{git shortlog -s -n -e}. We performed a de-duplication step based on the author names or email addresses. Figure \ref{fig:git_contribution_cdf} shows the total number of authors that contributed to the graph data in the legend. The number of de-duplicated authors is higher than the number of contributors we obtained from GitHub in \ref{tab:git_statistics}. We expect that GitHub users contributed to the repositories with different commit information. Following this logic the graphs in figure \ref{fig:plot_git_contribution_cdf} represents a lower estimate.


% \pb{Page views of ipfs.io}

% \pb{Traffic to go-ipfs}

% \pb{Number of contributions.}

% \pb{Distribution of contributions.}

% \pb{Evolution of IPFS.}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Content Publication Performance}
\label{sec:evaluation_content_publication_performance}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{plots/dht_pvdret_process_complete.pdf}
    \caption{CDFs for content publication (a--c) and content retrieval (d--f) for each AWS region that we employed for our lookup measurements. a) The overall publication duration that includes walking the DHT and then storing the provider record at appropriate peers. b) Only the just mentioned DHT walk c) Only the \texttt{ADD\_PROVIDER} RPCs. d) The overall content retrieval duration that includes walking the DHT and then fetching the data from the providing peer. e) Only the just mentioned DHT walk f) Only the fetch operation. This graph has a step shape due to the constant vantage points from where we were providing the content and the constant data size of the random data. The sample size is $4,324$ in all graphs across all AWS regions combined.}
    \label{fig:dht_pvdret_process_complete}
\end{figure*}

\begin{table}
    \centering
    \footnotesize
    \caption{Latency percentiles of the overall DHT publication and retrieval operations from different AWS regions.}
    \label{tab:dht_performance_percentiles}
    \vspace{-0.3cm}
    \begin{tabular*}{\linewidth}{l@{\extracolsep{\fill}}|rrr|rrr}
    \hline\hline
        \multicolumn{1}{c}{}        &          \multicolumn{3}{c}{Publication Percentiles}              &         \multicolumn{3}{c}{Retrieval Percentiles}            \\
        AWS Region                  & 50th                & 90th                 & 95th                 & 50th               & 90th              & 95th            \\ \hline
        \texttt{af\_south\_1}       & \SI{28.93}{\second} & \SI{107.14}{\second} & \SI{127.22}{\second} & \SI{2.82}{\second} & \SI{3.44}{\second} & \SI{3.67}{\second} \\
        \texttt{ap\_southeast\_2}   & \SI{36.26}{\second} & \SI{117.74}{\second} & \SI{142.79}{\second} & \SI{2.77}{\second} & \SI{3.44}{\second} & \SI{3.60}{\second} \\
        \texttt{eu\_central\_1}     & \SI{27.70}{\second} & \SI{106.91}{\second} & \SI{133.27}{\second} & \SI{1.67}{\second} & \SI{1.99}{\second} & \SI{2.09}{\second} \\
        \texttt{me\_south\_1}       & \SI{29.32}{\second} & \SI{105.45}{\second} & \SI{130.48}{\second} & \SI{2.10}{\second} & \SI{2.50}{\second} & \SI{2.61}{\second} \\
        \texttt{sa\_east\_1}        & \SI{42.32}{\second} & \SI{115.45}{\second} & \SI{148.04}{\second} & \SI{2.72}{\second} & \SI{3.22}{\second} & \SI{3.41}{\second} \\
        \texttt{us\_west\_1}        & \SI{36.02}{\second} & \SI{121.13}{\second} & \SI{147.59}{\second} & \SI{2.04}{\second} & \SI{2.46}{\second} & \SI{2.58}{\second} \\
    \hline\hline
    \end{tabular*}
\end{table}

As explained in Section \ref{sec:content-publication}, the content publication process consists of two steps. First, the content must be imported into the local IPFS node and second, provider records must be stored with suitable peers. The first (\ie importing content) step was covered by Lajam and Helmy \cite{LajamH21} in their performance analysis. Here, we focus on the advertisement of providers records.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\pb{Overall Delay.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Figure \ref{fig:dht_pvdret_process_complete}a, \ref{fig:dht_pvdret_process_complete}b and \ref{fig:dht_pvdret_process_complete}c show CDFs for the duration of the overall content publication process, the DHT walk to find suitable peers, and the \texttt{ADD\_PROVIDER} RPCs, respectively, for all provisioned AWS regions. 
We breakdown the results based on the region from which we publish the object. 

The publication process is significantly slower than that seen in more centralized stores, such as S3. 
The overall publication process across all regions takes \SI{33.8}{\second}, \SI{112.3}{\second} and \SI{138.1}{\second} in the 50th, 90th and 95th percentiles respectively.
Positively, we see similar results across all regions despite the larger build-up of presence in the US and China.
Table \ref{tab:dht_performance_percentiles} breaks down the publication duration percentiles for each AWS region individually.
Note, the kink at the \SI{50}{\second} mark in Figure \ref{fig:dht_pvdret_process_complete}a and \SI{45}{\second} mark in Figure \ref{fig:dht_pvdret_process_complete}b stems from an internal timeout.



%\gareth{I would remove the below stuff about termination and starvation. We don't seem to have any concrete results there, and this feels more like a design part of the paper. So, it doesn't really fit well here. Probably easiest just to remove}

%The breakdown also reveals the majority of time is spent in walking the DHT as opposed to storing the provider records. This is because of the DHT termination condition, whereby $k=20$ peers with the closest CID are queried, or all peers are queried (``starvation''). 



%The ``Starvation'' condition is more likely to occur only in small, e.g., private networks and not in the live public one which we can confirm as we have not observed queries contacting thousands of peers. Hence, IPFS stops searching for suitable peers only if it has asked, but not found, any closer ones from the set of closest peers it already knows. Due to the high churn rate (as shown in Section~\ref{sec:churn}), it is likely that intermediate peers during the DHT walk have stale records in their $k$-buckets pointing to peers that are not online anymore. Requests to those peers time out and delay the overall process.

\pb{Delay breakdown.}
After IPFS has found the closest peers it attempts to store provider records with them. It does so by first dialing to the $k=20$ closest (to the CID) peers (unless already connected) and then performing the \texttt{ADD\_PROVIDER} RPCs. It will not wait for a response from each peer, but will instead perform the RPCs in a ``fire and forget'' fashion.
\gareth{The above is more 'design' stuff that should be previously described. We shouldn't mix in new design details in the evaluation ideally.}
That said, \ref{fig:dht_pvdret_process_complete}c shows the CDFs for the overall duration of the batch of RPCs, instead of individual ones.
% from starting the first RPC until completion of the last. 
We find that  most of the times the IPFS node is not already connected to all of the 20 closest peers and therefore needs to dial it before performing the RPC. Further, some of those are often not reachable anymore and the dial attempts time out. Hence, the kinks in the graph depict various timeouts at different levels of the network stack which we will explain in the following paragraph.

There are steps at the \SI{5}{\second}, \SI{10}{\second}, \SI{15}{\second}, \SI{45}{\second}, \SI{50}{\second}, and \SI{60}{\second} mark. 
The kink at \SI{5}{\second} is related to dial timeouts on the transport level of the TCP\footnote{\url{https://github.com/libp2p/go-tcp-transport/blob/70d7181d07db9dd6b844d52ad01cf5b3182719ef/tcp.go\#L23}} and QUIC\footnote{\url{https://github.com/lucas-clemente/quic-go/blob/84e03e59760ceee37359688871bb0688fcc4e98f/internal/protocol/params.go\#L106}} implementations. 
The \SI{10}{\second} kink stems from the fact that IPFS dials eight addresses per peer concurrently, at most. If a peer record contains more than eight addresses and the peer is not reachable, IPFS runs in the \SI{5}{\second} timeout for the first eight addresses and then again for the remaining ones. This argument also holds true for the \SI{15}{\second} step, however, we have not observed peers with so many addresses. The reason is a timeout that is set at a higher level\footnote{\url{https://github.com/libp2p/go-libp2p-core/blob/ea6cbf9ff2894c96aa014006c475207e01d6780a/transport/transport.go\#L20}} and covers not only the dial itself but also the connection upgrade to a secure communication channel. The step at \SI{45}{\second} originates in the default handshake timeout of the Websocket\footnote{\url{https://github.com/gorilla/websocket/blob/9111bb834a68b893cebbbaed5060bdbc1d9ab7d2/client.go\#L142}} transport. Finally, the kink at \SI{60}{\second} is related to the maximum time for a single dial to a peer in \footnote{\url{https://github.com/libp2p/go-libp2p-core/blob/243f8b9e3c8185705c55510a8c15c65abee739f6/network/context.go\#L11}}. We have not found a reason for the step at the \SI{50}{\second} mark.



\yiannis{I think the description is also a bit verbose. Can someone take a stab at shortening it?}


\subsection{Content Retrieval Performance}

%The content routing process includes three steps: Content Discovery, Peer Discovery and Peer Routing. We next evaluate the performance of IPFS content retrieval. For the below consideration only the ``Content Discovery'' and ``Peer Routing'' procedures are relevant as in our measurement setup the provider records also contain the Multiaddresses to the providing peer which makes the ``Peer Discovery'' step obsolete.

We next evaluate the performance of IPFS content retrieval. 




\pb{Retrieval delay.}
Figures \ref{fig:dht_pvdret_process_complete}d, \ref{fig:dht_pvdret_process_complete}e and \ref{fig:dht_pvdret_process_complete}f show CDFs for the duration of the overall retrieval, the DHT walk to find provider record, and the final content fetch operation. 
Table~\ref{tab:dht_performance_percentiles} breaks down the retrieval duration percentiles for each AWS region individually.
We note that we experience a 100\% success rate, confirming the reliability our own deployment.
However, we experience notable performance diversity, with average delays significantly higher than typical webpage loading times. 
\gareth{Is there any way we could offer a baseline comparison?}
The performance difference is more pronounced among regions than in the publication process. 
For example, retrieval delays in central Europe are less than \SI{2}{\second} in \SI{90}{\percent} of the cases, compared to \SI{3.44}{\second} for Cape Town and Sydney.\footnote{Note, due to Bitswap, DHT queries are only launched after a timeout of 1s (see Section~\ref{sec:bitswap}).}
\gareth{Can we have some insight/quantification into why the region has an impact?}

%Note that all DHT walk operations only start after a \SI{1}{\second} delay as Figure \ref{fig:dht_pvdret_process_complete}e indicates. As explained in the Section~\ref{sec:bitswap}, IPFS tries to find content through Bitswap before sending \texttt{IWANT-HAVE} messages to all peers it is currently connected to. Only after a timeout of \SI{1}{\second} does it switch to the DHT content routing subsystem\footnote{\url{https://github.com/ipfs/go-bitswap/blob/dbfc6a1d986e18402d8301c7535a0c39b2461cb7/internal/defaults/defaults.go\#L10}}. We acknowledge that this is a potential avenue for optimization.

Each step in Figure \ref{fig:dht_pvdret_process_complete}f corresponds to a unique combination of our controlled providing IPFS instance and the respective retrieving one. Since the fetch duration includes the dial, protocol negotiation and data transmission times which are more or less constant among unique pairs of our controlled IPFS instances, it forms a step shape.
\gareth{Not sure I really understand what the previous paragraph is saying?}



\subsubsection{Churn}
\label{sec:churn}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{plots/crawl_churn_combined.pdf} 
    \caption{Churn rate as cumulative distribution functions. Each graph and line shows and  represents a subset of the \num{467134} session observations. The step shape correlates with the sampling interval of our crawler.}
    \label{fig:crawl_churn_combined}
\end{figure}

% go-ipfs (351,734)
% hydra-booster (29,929)
% storm (55,499)
% ioi (27,897)
% CN (119,899)
% US (51,996)
% DE (15,566)
% HK (81,404)
% BR (18,522)
% TW (28,115)

In this subsection we quantify the network churn for different subsets of peers by measuring the session lengths of all reachable peers in the network as described in Section~\ref{sec:methodology_network_crawls}. However, when measuring session lengths, we have to account for several statistical and systematic errors \cite{StutzbachR06}. Since we were monitoring all reachable peers and selected a time period for this analysis without any gaps in the data we avoid running the risk of a biased peer selection or missing data. Further, we follow the create-based method \cite{StutzbachR06, SaroiuGG, RoselliLA} for long session handling to minimize bias towards shorter sessions and account for peers that stay online beyond our selected measurement time window. Therefore, the graphs in Figure \ref{fig:crawl_churn_combined} are based on \num{467134} session observations in only the first half of our ``Detailed Analysis'' time window. All lines exhibit a step function shape due to the sampling interval of our monitor as outlined in section~\ref{sec:methodology_network_crawls}.

\gareth{Not sure how churn is relevant to performance? Is this not more about deployment? Or status quo? I reckon this needs placing elsewhere.}

Figure~\ref{fig:crawl_churn_combined}a shows churn rates for different IPFS agents and Figure \ref{fig:crawl_churn_combined}b shows churn rates for peers from different countries. For the latter we chose countries that stood out in the deployment analysis section~\ref{sec:deployment}. \hl{peers from DE least churn, as expected from the deployment section.}

% \dennis{Yiannis, could you cover the implications of the churn graphs?}
Peer churn is a very central characteristic of P2P networks. It affects the dynamicity of the network, as well as its operation. For this reason, there are specific settings in P2P protocols to account for nodes joining and leaving the network. For instance, the provider record replication setting, $k$, is there to account for churn. If $k$ is set too large, relative to the rate of nodes joining/leaving, then extra traffic is introduced to the network and extra resource requirements to peers themselves. The opposite, \ie a low $k$ value relative to churn, would result in unreachable content. The parameters discussed in Section \hl{XX} (\ie ``Re-publish interval" and ``Expiry interval") are set for this precise reason and seem to be accounting for the right rate of churn in the IPFS network, according to Figure~\ref{fig:crawl_churn_combined}.





\begin{itemize}
    \item relax the termination conditions for the content publication process (optimistic provide)
    \item Improvement suggestions: decrease find provider delay
    \item DHT 20 replication factor is appropriate given the churn
\end{itemize}




\pb{Retrieval Stretch.}
We next assess how well IPFS competes against HTTP. 
We measure this a stretch: the ratio of the IPFS retrieval time vs. the \textit{estimated} HTTP retrieval time. Specifically:

\begin{align}
    \mathrm{Stretch} &= \frac{\text{IPFS Content Retrieval Time}}{\text{HTTP Content Retrieval Time}} \\[0.2cm]
    & = \frac{\text{Discover} + \text{Dial} + \text{Negotiate} + \text{Fetch}}{\text{Dial} + \text{Negotiate} + \text{Fetch}}.
    \label{eq:definition_stretch}
\end{align}


\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{plots/dht_ret_stretch.pdf}
    \caption{CDFs of the stretch metric as it is defined in equation~\ref{eq:definition_stretch} for each AWS vantage point. The y-axis shows the fraction of retrieval operations that were totally performed from each AWS region. \SI{50}{\percent} of content retrieval operation performed took roughly $3.5$ times longer than the estimated corresponding HTTP request across all AWS regions.}
    \label{fig:dht_ret_stretch}
\end{figure}



%While we can equate the dial and fetch steps, there is uncertainty in how the negotiation and handshake steps relate to each other. Therefore, we only provide a lower bound measurement for the stretch metric by assuming that the IPFS protocol negotiation step is generally a more involved process than a TLS handshake. This can be made plausible by noting that the protocol negotiation step among other things involves the establishment of an encrypted communication channel as well. Hence, we define stretch as:



Figure~\ref{fig:dht_ret_stretch} a CDF for the stretch of all content retrieval operations for each AWS region. Almost every content retrieval operation took at least twice as long as the corresponding location-based request and $50\%$ of content retrieval operations took roughly $3.5$ times longer than the estimated corresponding HTTP request across all AWS regions. Note that the ``Discover'' step also includes the Bitswap delay mentioned in \hl{XY} because we want to compare the delays that the user would experience. \hl{say something about the (non)-difference between regions}
\yiannis{I believe we should add the benefits of content addressing for popular and widely cached content. I guess we can't show such results, but I think it's still worth it.}


\pb{Retrieval via Gateway.} 
It is worth noting that the content from the IPFS ecosystem can also be retrieved via the deployed public gateway and thus, gateways play a vital role in the deployments. We notice 6.57 TB of data transfer from the gateway. Gateways also have the capability to cache content items and can deliver them to the user. 
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{plots/gateway_response_details_v2.pdf} 
    \caption{Response from the gateways (a) Distribution of HTTP response codes (b) Distribution of upstream response latency (top X2-axis) and bytes downloaded per request to the gateway from peers (bottom X-axis)}
    \label{fig:gateway_response_time}
\end{figure}

We proceed to study the retrieval latencies of files to the gateway from the peers.  Looking at the response status code (Figure~\ref{fig:gateway_response_time}a), we see that only 64.9\% of requests were successful, with the http status code 200 or 206, delivering 94.8\% of total bytes. 14.8\% of requests were merely redirects (status code 301) to the correct subdomain version to ensure any encoding conversions, for example, content representation identifier from v1 to v2.   Interestingly, for 16.16\% of requests, we find clients terminating the connection with the gateway even before the content is served. We believe that the reason for this connection abortion is related to the response latency, thereby affecting the overall user experience. 

As such the response latency is built by two factors, \one latency between the client device and the gateway, as commonly noticed in any kind of client-server communications and \two latency between the gateway and the peer serving the content, which is innate to IPFS gateways. Figure~\ref{fig:gateway_response_time}b (X2 axis) shows the impact of the second factor for the successful requests. 46\% of the requests are served by the gateway-cache, serving close to 50\% of the total traffic. From the remaining, 76.03\% of the requests are delivered in less than 250ms and less than 1\% has a latency of more than 10 seconds. We find the median response size is 664.59 KB, but there is no correlation between the response size and the latency (Pearson correlation coefficient of 0.13). 


\subsection{Overhead}
\label{sec:overhead}

\pb{Routing Table Maintenance.}

- number of provider records
- number of peer records

\pb{Routing overhead}
Best path vs actual path. Talking as the baseline the path between the location of the request and the location of the closest node with content, we compare it with the actual path.





\subsection{Limitations}


% \subsection{Gateway Data}
% From PL:
% \begin{itemize}
%     \item number of peers per gateway, possibly for a few gateways only (grafana)
%     \item Wantlist length (grafana)
%     \item number of peerings (?) (grafana)
%     \item peers by transport (?) (grafana)
%     \item number of server vs client nodes
%     \item NAT'ed vs non-NAT'ed nodes - \textbf{How do we find that?}
%     \item Server Load: CPU Seconds (?), Memory, Open FDs, (goroutines?) (grafana)
%     \item Bandwidth Requirement per gateway (grafana)
%     \item Measurements: Lots of new things to add - \textbf{Is that not the subject of the next section?}
%     \item Hydra boosters. If we include description of Hydras, there are lots of graphs we can include from grafana. \textbf{That assumes we get data from Hydra's, right? Is there something we can measure ourselves?}
% \end{itemize}

% \subsection{Measurement Data}
% \subsubsection{Nebula}
% \begin{itemize}
%     \item Churn
%     \item Inter Arrival Times
%     \item Node Geo Locations
%     \item numbers about the network size
%     \item Fraction of nodes on cloud infrastructure
%     \item Agent versions in use in the IPFS network.
%     \item IPv4 vs IPv6 usage
%     \item Number of unique IP-addresses in use
%     \item Number of nodes providing relaying services
%     \item Ping latency from the Nebula running node to all other nodes in the DHT
% \end{itemize}

% \subsubsection{DHT Lookup Latency}

% \begin{itemize}
%     \item Lookup latency histogram
%     \item Provide latency histogram
%     \item Storm node insights
%     \item Latency map
% \end{itemize}


% \subsection{Public Data}
% From GitHub:

% \begin{itemize}
%     \item Stars (Star gazer chart? https://github.com/caarlos0/starcharts)
%     \item Contributors
%     \item Forks
%     \item Commits
%     \item LoC
% \end{itemize}

